Don't Look into the Dark: Latent Codes for Pluralistic Image Inpainting

We present a method for large-mask pluralistic image inpainting based on the generative framework of discrete latent codes. Our method learns latent priors, discretized as tokens, by only performing computations at the visible locations of the image. This is realized by a restrictive partial encoder that predicts the token label for each visible block, a bidirectional transformer that infers the missing labels by only looking at these tokens, and a dedicated synthesis network that couples the tokens with the partial image priors to generate coherent and pluralistic complete image even under extreme mask settings. Experiments on public benchmarks validate our design choices as the proposed method outperforms strong baselines in both visual quality and diversity metrics.

==> macro.tex <==

\newcommand{\PreserveBackslash}[1]{\let\temp=\\#1\let\\=\temp}
%\newcolumntype{C}[1]{>{\PreserveBackslash\centering}p{#1}}

%% the following commands are plagiarized from Ravi
\newcommand{\pcline }{\rule{1in}{0.0in}    }  % Spacing for pseudo-code.
\newcommand{\pctab  }{\hspace{0.10in}      }  % Pseudo-code indentation.
\newcommand{\pcbigtab  }{\hspace{1.75in}    }  % Pseudo-code indentation.
\newcommand{\pcasgn }{\mbox{$\leftarrow$}  }  % Pseudo-code assignment operator
%%\newcommand{\pcgreater}{\mbox{$\leftarrow$} } % Pseudo-code bigger operator
\newcommand{\pcomment}[1]{\mbox{// {\it #1}}}  % Pseudo-code comments.
\newcommand{\pckeyword}[1]{\mbox{{\bf #1}}}  % Pseudo-code keywords.
\newcommand{\pcspace}{\hspace{0.10in}}

\newcommand{\pcode}[1]{
	\footnotesize
	\vspace{-0.1in}
	\begin{minipage}{100in} % The width argument will be ignored:
		% See lamport p. 99
		\begin{tabbing} \hspace{0.10in} \= \pctab \= \pctab \= \pctab \= \pcbigtab \= \\
			#1
		\end{tabbing}
	\end{minipage}
	%    \vspace{0.15in}
}
%% enf of the pseudo code environment

\newcommand{\tabtextsize}{\small}
\newcommand{\figtext}[1]{{\footnotesize #1}}
%%\newcommand{\Caption}[1]{\caption{\small {\em #1}}}
%%\newcommand{\Caption}[1]{\caption{{\em #1}}}
\newcommand{\Caption}[2]{\caption[#1]{{\footnotesize #1} {\footnotesize #2}}}
%%\newcommand{\Caption}[1]{\caption{\it \small {#1}}}

\newcommand{\invisible}[1]{{\color{white} #1}}
\newcommand{\emacsquote}[1]{{``#1''}}

\newcommand{\revision}[1]{{\color{blue} #1}}

\definecolor{DeltaColor}{rgb}{0.039,0.73,0.71}
\definecolor{SetaColor}{rgb}{0.867, 0.0235, 0.376}
\definecolor{SigmaColor}{rgb}{0.98,0.45,0.0}
\definecolor{RedColor}{rgb}{0.8,0,0}
\definecolor{AlphaColor}{rgb}{0,0,0.8}
\definecolor{BetaColor}{rgb}{0.8,0,0.8}
\definecolor{GammaColor}{rgb}{0.5,0,0.7}
\definecolor{EpsilonColor}{rgb}{0.353,0.725,0.906}
\definecolor{TauColor}{rgb}{0.423,0.235,0.192}
\newcommand{\haiwei}[1]{{\color{AlphaColor} Haiwei: #1 $\qed$}}
\newcommand{\yajie}[1]{{\color{GammaColor} Yajie: #1 $\qed$}}
\newcommand{\gonglin}[1]{{\color{GammaColor} Gonglin: #1 $\qed$}}


\newcommand{\warning}[1]{{\it\color{red} #1}}
\newcommand{\Note}[1]{{\it\color{blue} #1}}
\newcommand{\nothing}[1]{}
\newcommand{\passthrough}[1]{#1}
\definecolor{AudioColor}{rgb}{0.56,0.34,0.62}
\newcommand{\audio}[1]{{\color{AudioColor} Audio: #1}}

\definecolor{DeadlineColor}{rgb}{0.9,0.4,0} % energetic color
\newcommand{\deadline}[1]{{\bf\color{DeadlineColor} ETA: #1}}

\newcommand{\psdraftboxDefault}{\psnodraftbox}

\definecolor{figred}{rgb}{1,0,0}
\definecolor{figgreen}{rgb}{0,0.6,0}
\definecolor{figblue}{rgb}{0,0,1}
\definecolor{figpink}{rgb}{1,0.63,0.63}

%\renewcommand{\warning}[1]{}

% \ifthenelse{\equal{\final}{1}}
% {
% 	\renewcommand{\weikai}[1]{}
% 	\renewcommand{\haiwei}[1]{}
% 	\renewcommand{\shichen}[1]{}
% 	\renewcommand{\hao}[1]{}
% 	\renewcommand{\Note}[1]{}
% }
% {}

\newcommand{\pseudocode}{Pseudocode}
\newcounter{pccount}
\setcounter{pccount}{1}
\newcommand{\pccaption}[1]{\textbf{Pseudocode \thepccount \hspace{0.5em}} #1 \addtocounter{pccount}{ 1}}

\newcommand{\algoname}[1]{\textnormal{\textsc{#1}}}

% \floatstyle{plain}
%\newfloat{algorithm}{tbhp}{lop}
%\floatname{algorithm}{\pseudocode}

\newcommand{\filename}[1]{\url{#1}}
\newcommand{\foldername}[1]{\url{#1}}
\newcommand{\bloginput}[1]{\input{blog/#1}}
\newcommand{\oldinput}[1]{\input{old/#1}}

\DeclareMathOperator*{\argmin}{argmin}         % for argmin or argmax equations
%\renewcommand{\algorithmicrequire}{\textbf{Input:}}   %Use Input in the format of Algorithm
%\renewcommand{\algorithmicensure}{\textbf{Output:}}  % UseOutput in the format of Algorithm




